Video-based Point Cloud Compression Artifact Removal

Photo-realistic point cloud capture and transmission are the fundamental enablers for immersive visual communication. The coding process of dynamic point clouds, especially video-based point cloud compression (V-PCC) developed by the MPEG standardization group, is now delivering state-of-the-art performance in compression efficiency. V-PCC is based on the projection of the point cloud patches to 2D planes and encoding the sequence as 2D texture and geometry patch sequences. However, the resulting quantization errors from coding can introduce compression artifacts, which can be very unpleasant for the quality of experience (QoE). In this work, we developed a novel out-of-the-loop point cloud geometry artifact removal solution that can significantly improve reconstruction quality without additional bandwidth cost. Our novel framework consists of a point cloud sampling scheme, an artifact removal network, and an aggregation scheme. The point cloud sampling scheme employs a cube-based neighborhood patch extraction to divide the point cloud into patches. The geometry artifact removal network then processes these patches to obtain artifact-removed patches. The artifact-removed patches are then merged together using an aggregation scheme to obtain the final artifact-removed point cloud. We employ 3D deep convolutional feature learning for geometry artifact removal that jointly recovers both the quantization direction and the quantization noise level by exploiting projection and quantization prior. The simulation results demonstrate that the proposed method is highly effective and can considerably improve the quality of the reconstructed point cloud.

==> authors_bio_portrait/Anique_Akhtar_bio.tex <==
\begin{IEEEbiography}
[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{../figure/Anique_Akhtar_portrait.jpg}}]{Anique Akhtar} received his B.S. degree in Electrical Engineering from Lahore University of Management Sciences (LUMS), Lahore, Pakistan, in 2013, and the M.S. degree from Koc University, Istanbul, Turkey, in 2015. He is currently pursuing his Ph.D. at University of Missouri-Kansas City (UMKC). He has worked on wireless communication in the past and is currently working at the multimedia and communications lab. His research interests include point cloud compression and communication, and deep learning solutions for point cloud processing.\end{IEEEbiography}

==> authors_bio_portrait/Li_Li_bio.tex <==
\begin{IEEEbiography}
[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{../figure/Li_Li_portrait.eps}}]{Li Li} (M'17) is a research fellow with department of electronic engineering and information science, University of Science and Technology of China (USTC).
He received the B.S. and Ph.D. degrees in electronic engineering from USTC, Hefei, Anhui, China, in 2011 and 2016, respectively.
He was a visiting assistant professor in University of Missouri-Kansas City from 2016 to 2020.
His research interests include image/video coding and processing.
He received the Best 10\% Paper Award at the 2016 IEEE Visual Communications and Image Processing (VCIP) and the 2019 IEEE International Conference on Image Processing (ICIP).
\end{IEEEbiography}

==> authors_bio_portrait/Shan_Liu_bio.tex <==
\begin{IEEEbiography}
[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{../figure/Shan_Liu_portrait.jpg}}]{Shan Liu} received the B.Eng. degree in Electronic Engineering from Tsinghua University, the M.S. and Ph.D. degrees in Electrical Engineering from the University of Southern California, respectively. She is currently a Tencent Distinguished Scientist and General Manager of Tencent Media Lab. She was formerly Director of Media Technology Division at MediaTek USA. She was also formerly with MERL and Sony, etc. Dr. Liu has been actively contributing to international standards since the last decade and served co-Editor of H.265/HEVC SCC and H.266/VVC. She has numerous technical proposals adopted into various standards, such as VVC, HEVC, OMAF, DASH, MMT and PCC, etc. Technologies and products developed by her and under her leadership have served hundreds of millions of users. Dr. Liu holds more than 200 granted US and global patents and has published more than 100 journal and conference papers. She was in the committee of Industrial Relationship of IEEE Signal Processing Society (2014-2015). She served the VP of Industrial Relations and Development of Asia-Pacific Signal and Information Processing Association (2016-2017) and was named APSIPA Industrial Distinguished Leader in 2018. She is on the Editorial Board of IEEE Transactions on Circuits and Systems for Video Technology (2018-present) and received the Best AE Award in 2019 and 2020, respectively. She also served or serves as a guest editor for a few T-CSVT special issues and special sections. She has been serving Vice Chair of IEEE Data Compression Standards Committee since 2019. Her research interests include audio-visual, volumetric, immersive and emerging media compression, intelligence, transport and systems.
\end{IEEEbiography}

==> authors_bio_portrait/Wei_Jia_bio.tex <==
\begin{IEEEbiography}
[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{../figure/Wei_Jia_portrait.jpg}}]{Wei Jia} is a Ph.D. candidate with department of computer science electrical engineering, University of Missouri-Kansas City (UMKC).
He received the B.S. and M.S. degrees in electronic engineering from Beijing University of Posts and Telecommunications (BUPT), Beijing, China, in 2009 and 2012, respectively.
His research interests include image/video coding and processing, video-based point cloud compression, and deep learning.
\end{IEEEbiography}

==> authors_bio_portrait/Wen_Gao_bio.tex <==
\begin{IEEEbiography}
[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{../figure/Wen_Gao_portrait.jpg}}]{Wen Gao} received the B.Eng. degree from University of Science and Technology of China, the M.S. degree from Peking University and Ph.D. degrees from Purdue University, all in Electrical Engineering. He is currently a Principal Researcher of Tencent Media Lab. He was formerly a senior staff software engineer/manager in Harmonic Inc, and a principal scientist/manager in Princeton Research Lab of Technicolor Inc. He has multiple years of research and development experience in video compression and wireless communications. He made contributions to variety of standard organizations such as MPEG, AVS, 3GPP, ATSC, DVB and IEEE802 standard committees, etc. His current research interests are in the areas of point cloud compression, video coding for machines and machine learning. 
\end{IEEEbiography}

==> authors_bio_portrait/Zhu_Li_bio.tex <==
\begin{IEEEbiography}
[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{../figure/zhu_li_portrait.jpg}}]{Zhu Li} is now an Associate Professor with the Dept of Computer Science \& Electrical Engnieering (CSEE), University of Missouri,Kansas City, and director of the NSF I/UCRC Center for Big Learning (CBL) at UMKC. He received his PhD in Electrical \& Computer Engineering from Northwestern University, Evanston in 2004. He was AFOSR SFFP summer visiting faculty at the US Air Force Academy (USAFA), 2016 , 2017 , 2018 and 2020. He was Sr. Staff Researcher/Sr. Manager with Samsung Research America's Multimedia Standards Research Lab in Richardson, TX, 2012-2015, Sr. Staff Researcher with FutureWei (Huawei) Technology's Media Lab in Bridgewater, NJ, 2010~2012, an Assistant Professor with the Dept of Computing, The Hong Kong Polytechnic University from 2008 to 2010, and a Principal Staff Research Engineer with the Multimedia Research Lab (MRL), Motorola Labs, from 2000 to 2008. His research interests include point cloud and light field compression, graph signal processing and deep learning in the next gen visual compression, image processing and understanding. He has 47 issued or pending patents, 160+ publications in book chapters, journals, and conferences in these areas. He is an IEEE senior member, Associate Editor-in-Chief for IEEE Trans on Circuits \& System for Video Tech, associated editor for IEEE Trans on Image Processing(2020~), IEEE Trans.on Multimedia (2015-18), IEEE Trans on Circuits \& System for Video Technology(2016-19). He serves on the steering committee member of IEEE ICME (2015-18), he is an elected member of the IEEE Multimedia Signal Processing (MMSP), IEEE Image, Video, and Multidimensional Signal Processing (IVMSP), and IEEE Visual Signal Processing \& Communication (VSPC) Tech Committees. He is program co-chair for IEEE Int’l Conf on Multimedia \& Expo (ICME) 2019, and co-chaired the IEEE Visual Communication \& Image Processing (VCIP) 2017.  He received the Best Paper Award at IEEE Int'l Conf on Multimedia \& Expo (ICME), Toronto, 2006, the Best Paper Award (DoCoMo Labs Innovative Paper) at IEEE Int'l Conf on Image Processing (ICIP), San Antonio, 2007.
\end{IEEEbiography}
